Luring of transferable adversarial perturbations in the black-box paradigm

The growing interest for adversarial examples, i.e. maliciously modified examples which fool a classifier, has resulted in many defenses intended to detect them, render them inoffensive or make the model more robust against them. In this paper, we pave the way towards a new approach to improve the robustness of a model against black-box transfer attacks. A removable additional neural network is included in the target model, and is designed to induce the \textit{luring effect}, which tricks the adversary into choosing false directions to fool the target model. Training the additional model is achieved thanks to a loss function acting on the logits sequence order. Our deception-based method only needs to have access to the predictions of the target model and does not require a labeled data set. We explain the luring effect thanks to the notion of robust and non-robust useful features and perform experiments on MNIST, SVHN and CIFAR10 to characterize and evaluate this phenomenon. Additionally, we discuss two simple prediction schemes, and verify experimentally that our approach can be used as a defense to efficiently thwart an adversary using state-of-the-art attacks and allowed to perform large perturbations.

==> background.tex <==
In this section we introduce some notations and provide background about adversarial attacks in a black-box setting.

\subsection{Notations}
We consider a classification task where input-label pairs $(x,y) \in \mathcal{X} \times \mathcal{Y}$ (with $\mid\mathcal{Y}\mid = C$) are sampled from a distribution $\mathcal{D}$. A neural network model $M_\theta : \mathcal{X} \rightarrow \mathcal{Y}$, classifies an input  $x \in \mathcal{X}$ to a label $M(x) \in \mathcal{Y}$. 
$\mathcal{L}\big(M_\theta(x),y\big)$ is the cross-entropy loss for $M_\theta$ with respect to an input $x\in\mathcal{X}$ and the ground-truth label $y \in \mathcal{Y}$.
The pre-softmax function of $M_\theta$ (the logits) is denoted as $\ell: \mathcal{X} \rightarrow \mathbb{R}^C$. For the sake of readability, the model $M_\theta$ is simply noted as $M$, except when necessary. 

\subsection{Adversarial examples in the black-box setting}
When the adversary is in a white-box setting, therefore allowed to compute gradients, he can use one of the many existing \textit{gradient-based} attacks \citep{goodfellow2015laceyella, carlini2017towards, chen2018ead, Dong_2018, Madry2017,  wang2019enhancing}. Whenever the adversary is in a black-box setting, paradigm, only allowed to get the output label or output confidence score from the target model, he can still use gradient-free methods to mount an adversarial attack \citep{uesato2018adversarial, guo2019simple, su2019one, brendel2017decision, ilyas2018black, chen2019boundary}.
However, the number of queries requires to mount the attack is prohibitive in a real-world setting and may be flagged as suspicous \citep{chen2019stateful, li2020blacklight}.
In that case, the adversary can rely on the phenomenon of transferability of adversarial examples \citep{papernot2017practical}.%: adversarial examples crafted on a model will potentially fool another model trained for the same task. 
Practically, the adversary trains his own substitute model, crafts adversarial examples on it, and transfers them to the target model. 


\begin{comment}
\paragraph{Adversarial attacks used.}
We present here the five attack methods used throughout the paper. We detail them in their untargeted and $l_{\infty}$ version, meaning that no particular label different from the ground-truth is targeted, and that the $l_{\infty}$ norm of the adversarial perturbation is upper-bounded by $\epsilon$.
We note $x'$ the adversarial example crafted from a well-classified clean example $x$ of ground-truth label $y$, and  $J$ designates the cross-entropy loss.\\
\textbf{FGSM} attack \citep{goodfellow2015laceyella} aims at minimizing $J(\theta, x + \alpha,y) - J(\theta,x,y)$ with respect to $\alpha$, given that $\left\| \alpha \right\|_{\infty} < \epsilon$. A linear approximation yields:
\begin{align}
    x' = x + \epsilon sign\big( \nabla_x J(\theta,x_n,y)\big)
\end{align}
At the end, clipping is performed to respect possible box constraints (e.g. the pixels values may have to keep in a certain range).\\
\textbf{PGD}~\citep{Madry2017} is an iterative version of FGSM, with clipping performed at each step, and an additional random step performed at the beginning for better convergence:
\begin{align}
    \begin{split}
    x'_0 & = Clip_{B_{\infty}(x, \epsilon)} (x + r) \\
    x'_{n+1} & = Clip_{B_{\infty}(x, \epsilon)}(x'_n + \alpha sign\big( \nabla_x J(\theta,x_n,y)\big)
    \end{split}
\end{align}
where $B_{\infty}(x, \epsilon)$ is the $l_{\infty}$-ball of radius $\epsilon$ and center $x$, $\alpha$ the step size and $r$ the initial random-step.\\
\textbf{MIM}~\citep{Dong_2018} is a modified version of the PGD attack, designed for transferability purpose. This attack is based on the intuition that adding a momentum term to the gradient leads to more consistent (i.e in the same direction) updates throughout the attack and accelerates the convergence:
\begin{align}
    \begin{split}
    x'_{n+1} = &  Clip_{B_{\infty}(x, \epsilon)} \big(x'_n + \alpha sign(g_{n+1})\big) \\
    g_n = & \nabla_x J(\theta,x_n,y) \\
    g_{n+1} & = \mu g_n + \frac{\nabla_x J(\theta,x_n,y)}{\left\| \nabla_x J(\theta,x_n,y) \right\|_1}
    \end{split}
\end{align}
where $\mu$ is the decay factor.\\
\textbf{MIM-TI} attack \citep{Dong2019EvadingDT} is an enhanced version of MIM focused on better transferability properties. The gradient of the loss is convolved with a kernel matrix to simulate computing gradients on translated images. The intuition behind this is to take into account that the source and the target networks rely on different regions on the input space to perform prediction. \\
\textbf{DIM}~\citep{Xie2018ImprovingTO} is another enhanced version of MIM. At each step of the attack, with probability $p$,  the input is transformed with image resizing or random padding in order to reduce possible overfitting effects.\\
\textbf{DIM-TI}~\citep{Dong2019EvadingDT} encompasses the MIM-TI and DIM attacks.
\end{comment}


\begin{comment}

\subsection{Defense methods}
\label{defense_sota}

To protect a model against adversarial examples, many methods have been investigated, which mainly focus on the white-box setting where the adversary has a complete knowledge of the target model.
\textbf{Proactive defenses.} aim at making the model intrinsically robust to adversarial examples, by relying on a specific training procedure \citep{Madry2017, kannan2018adversarial, zhang2019theoretically}, specific activation functions or specific inference schemes \citep{dhillon2018stochastic, taghanaki2019kernelized, Xiao2020Enhancing}.
\textbf{Purification methods.} consist in mitigating the adversarial perturbation from the input before it is fed to the target model \citep{xu2017feature, buckman2018thermometer, hwang2019puvae, Xie_2019_CVPR}.
%Considering an adversarial example $x'$ crafted from a clean example $x$ to fool a target model $M$ (i.e. $M(x') \neq y$), a purification method aims at designing a denoiser $D$, such that $D(x') \approx x$ and then $M\big(D(x')\big) = y$.
\textbf{Detection methods.} detect an adversarial example with methods mainly based on the assumption that clean and adversarial data belong to different manifolds \citep{grosse2017statistical, zheng2018robust, metzen2017detecting, samangouei2018defense, meng2017magnet}. These approaches develop statistical tests or rely on specific detection mechanisms. 
%Whereas purification methods are designed to  retrieve the true label, many detection mechanisms only raise a flag when an adversarial example is detected.
Purification and detection methods are considered as \textit{reactive defense} schemes, as they consider an already trained model and try to protect it against adversarial examples. %These methods often consider a gray-box setting where the adversary is not aware of the presence of the defense mechanism. 
However, these methods have been shown to be easily bypassed or to focus only against specific adversarial perturbations \citep{carlini2017adversarial, athalye2018robustness}.
\textbf{Provable methods.} aim at giving robustness certificates to the defender. Considering a clean example $x$, a certificate allows the defender to know if an adversarial example can be found at some distance $d$ (called \textit{certificate value}) of $x$ \citep{cohen2019certified,raghunathan2018certified,kolter2017provable,gowal2018effectiveness}.
%Most of these approaches employ convex relaxations to compute a lower-bound of the minimal adversarial perturbation needed to turn $x$ into an adversarial example 
\end{comment}




==> cifar10_table_AC_DAC.tex <==
\begin{table*}[t]
\caption{CIFAR10. $\text{AC}_{MoP}$, $\text{AC}_M$ and
DAC for different source model architectures.}
\label{CIFAR10 final results}
\vskip 0.15in
\begin{center}
%\begin{small}
\begin{sc}
\resizebox{0.83\linewidth}{!}{
%\footnotesize
\begin{tabular}{ccccc|ccc|ccc}
%\hline
%& & \multicolumn{9}{c}{Architectures}\\
\hline
& & \multicolumn{3}{|c}{Stack} & \multicolumn{3}{|c}{C\_E} & \multicolumn{3}{|c}{Luring} \\
\hline
& \multicolumn{1}{c|}{$\epsilon$} & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC \\
\hline
SPSA
& \multicolumn{1}{|c|}{0.02} & 0.01 & 0.75 & 0.78 & 0.06 & 0.68 & 0.71 & 0.12 & \textbf{0.78} & \textbf{0.82} \\
& \multicolumn{1}{|c|}{0.03} & 0.0 & 0.57 & 0.62 & 0.01 & 0.45 & 0.49 & 0.02 & \textbf{0.59} & \textbf{0.64} \\
& \multicolumn{1}{|c|}{0.04} & 0.0 & 0.38 & 0.42 & 0.0 & 0.22 & 0.24 & 0.01 & \textbf{0.42} & \textbf{0.50} \\
\hline
ECO
& \multicolumn{1}{|c|}{0.02} & 0.15 & 0.7 & 0.71 & 0.14 & 0.6 & 0.63 & 0.16 & \textbf{0.81} & \textbf{0.87} \\
& \multicolumn{1}{|c|}{0.03} & 0.09 & 0.44 & 0.59 & 0.09 & 0.36 & 0.42 & 0.2 & \textbf{0.65} & \textbf{0.67} \\
& \multicolumn{1}{|c|}{0.04} & 0.05 & 0.29 & 0.29 & 0.04 & 0.28 & 0.34 & 0.09 & \textbf{0.35} & \textbf{0.44} \\
\hline
MIM-W
& \multicolumn{1}{|c|}{0.02} & 0.0 & 0.49 & 0.52 & 0.02 & 0.4 & 0.43 & 0.03 & \textbf{0.58} & \textbf{0.64} \\
& \multicolumn{1}{|c|}{0.03} & 0.0 & 0.24 & 0.28 & 0.0 & 0.15 & 0.19 & 0.0 & \textbf{0.30} & \textbf{0.39} \\
& \multicolumn{1}{|c|}{0.04} & 0.0 & 0.13 & 0.16 & 0.0 & 0.05 & 0.1 & 0.0 & \textbf{0.18} & \textbf{0.28} \\
\hline
\end{tabular}
%\normalsize
}
\end{sc}
%\end{small}
\end{center}
\end{table*}

==> figure_l0_distortion.tex <==
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.7\linewidth]{fig/hist_l0_mnist_cifar10.pdf}}  
\caption{$l_0$ distortion between clean and adversarial examples, depending on the architecture, for MNIST (left) and CIFAR10 (right)}
\label{hist_l0}
\end{center}
\end{figure}

==> figure_saliency_maps.tex <==
\begin{figure}[t-]
\begin{center}
\centerline{\includegraphics[width=0.5\linewidth]{fig/example_mnist_grad.pdf}}  
\caption{Saliency maps for MNIST. Top: clean image, $\nabla_{x}{\mathcal{L}(M(x),y)}$. Bottom: $\nabla_{x}{P(x)} $ for 3 augmented models.}
\label{example_mnist_grad}
\end{center}
\end{figure}

==> svhn_table_AC_DAC.tex <==
\begin{table*}[t]
\caption{SVHN. $\text{AC}_{MoP}$, $\text{AC}_M$ and 
DAC for different source model architectures.}
\label{SVHN final results}
\vskip 0.15in
\begin{center}
%\footnotesize
%\begin{small}
\begin{sc}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc|ccc|ccc|ccc}
%\hline
%& & \multicolumn{12}{c}{Architectures}\\
\hline
& & \multicolumn{3}{|c}{Stack} & \multicolumn{3}{|c}{Auto} & \multicolumn{3}{|c}{C\_E} & \multicolumn{3}{|c}{Luring} \\
\cline{3-14}
& \multicolumn{1}{c|}{$\epsilon$} & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC \\
\hline
SPSA
& \multicolumn{1}{|c|}{0.03} & 0.10 & 0.54 & 0.56 & 0.06 & 0.37 & 0.38 & 0.06 & 0.67 & 0.68 & 0.0 & \textbf{0.96} & \textbf{0.97} \\
& \multicolumn{1}{|c|}{0.06} & 0.01 & 0.21 & 0.24 & 0.0 & 0.10 & 0.11 & 0.0 & 0.37 & 0.42 & 0.0 & \textbf{0.96} & \textbf{0.96} \\
& \multicolumn{1}{|c|}{0.08} & 0.0 & 0.13 & 0.15 & 0.0 & 0.06 & 0.06 & 0.0 & 0.23 & 0.28 & 0.0 & \textbf{0.94} & \textbf{0.96} \\
\hline
ECO
& \multicolumn{1}{|c|}{0.03} & 0.06 & 0.42 & 0.44 & 0.14 & 0.48 & 0.49 & 0.18 & 0.66 & 0.68 & 0.20 & \textbf{0.97} & \textbf{0.98} \\
& \multicolumn{1}{|c|}{0.06} & 0.0 & 0.11 & 0.12 & 0.06 & 0.09 & 0.11 & 0.1 & 0.35 & 0.39 & 0.1 & \textbf{0.86} & \textbf{0.88} \\
& \multicolumn{1}{|c|}{0.08} & 0.0 & 0.03 & 0.07 & 0.06 & 0.09 & 0.09 & 0.08 & 0.29 & 0.32  & 0.09 & \textbf{0.84} & \textbf{0.86} \\
\hline
MIM-W
& \multicolumn{1}{|c|}{0.03} & 0.04 & 0.32 & 0.35 & 0.01 & 0.20 & 0.21 & 0.03 & 0.41 & 0.45 & 0.11 & \textbf{0.81} & \textbf{0.87} \\
& \multicolumn{1}{|c|}{0.06} & 0.0 & 0.06 & 0.09 & 0.0 & 0.03 & 0.05 & 0.0 & 0.10 & 0.18 & 0.0 & \textbf{0.58} & \textbf{0.71} \\
& \multicolumn{1}{|c|}{0.08} & 0.0 & 0.03 & 0.06 & 0.0 & 0.01 & 0.02 & 0.0 & 0.06 & 0.13 & 0.0 & \textbf{0.48} & \textbf{0.67} \\
\hline
\end{tabular}
}
\end{sc}
%\end{small}
%\normalsize
\end{center}
\end{table*}

==> table_trapdoor_short.tex <==
\begin{table}[t]
\caption{Worst $\text{AC}_{MoP}$, $\text{AC}_M$ and DAC values (MIM, DIM, MIM-TI and DIM-TI) for the Trapdoor and Luring approaches.}
\label{trapdoor_results}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\footnotesize
\begin{tabular}{p{1.2cm}p{0.5cm}p{0.7cm}p{0.4cm}p{0.5cm}|p{0.7cm}p{0.4cm}p{0.5cm}}
%\hline
%& & \multicolumn{6}{c}{Method}\\
\hline
& & \multicolumn{3}{|c}{Trapdoor} & \multicolumn{3}{|c}{Luring} \\
\hline
& \multicolumn{1}{c|}{$\epsilon$} & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC & $\text{AC}_{MoP}$ & $\text{AC}_{M}$ & DAC \\
\hline
MNIST
%& \multicolumn{1}{|c|}{0.2} & 0.06 & 0.82 & \textbf{0.97} & 0.19 & \textbf{0.92} & 0.93 \\
& \multicolumn{1}{|c|}{0.3} & 0.0 & 0.54 & \textbf{0.94} & 0.13 & \textbf{0.69} & 0.75 \\
%& \multicolumn{1}{|c|}{0.4} & 0.0 & 0.27 & \textbf{0.87} & 0.07 & \textbf{0.34} & 0.45 \\
\hline
SVHN
%& \multicolumn{1}{|c|}{0.03} & 0.1 & 0.48 & 0.58 & 0.11 & \textbf{0.81} & \textbf{0.87} \\
& \multicolumn{1}{|c|}{0.06} & 0.07 & 0.38 & 0.48 & 0.0 & \textbf{0.58} & \textbf{0.71} \\
%& \multicolumn{1}{|c|}{0.08} & 0.01 & 0.23 & 0.38 & 0.0 & \textbf{0.48} & \textbf{0.67} \\
\hline
CIFAR10
%& \multicolumn{1}{|c|}{0.02} & 0.0 & \textbf{0.71} & \textbf{0.84} & 0.03 & 0.58 & 0.64 \\
& \multicolumn{1}{|c|}{0.03} & 0.0 & \textbf{0.58} & \textbf{0.77} & 0.0 & 0.30 & 0.39 \\
%& \multicolumn{1}{|c|}{0.04} & 0.0 & \textbf{0.45} & \textbf{0.78} & 0.0 & 0.16 & 0.27 \\
\hline
\end{tabular}
\normalsize
\end{sc}
\end{small}
\end{center}
\end{table}

==> threat_model_figure.tex <==
%\begin{figure*}[t!]
%\begin{center}
%\centerline{\includegraphics[width=0.9\linewidth]{fig/use_case.pdf}}  
%\caption{A use-case illustrating the threat model. An API provider uses our defense scheme to release a public version of a model with minimal risk of transferability from the public model to the private API.}
%\label{use_case}
%\end{center}
%\end{figure*}
